AppBench: Planning of Multiple APIs from Various APPs for Complex User Instruction

Large Language Models (LLMs) can interact with the real world by connecting with versatile external APIs, resulting in better problem-solving and task automation capabilities. Previous research primarily focuses on APIs with limited arguments from a single source or overlooks the complex dependency relationship between different APIs. However, it is essential to utilize multiple APIs collaboratively from various sources (e.g., different Apps in the iPhone), especially for complex user instructions. In this paper, we introduce \texttt{AppBench}, the first benchmark to evaluate LLMs' ability to plan and execute multiple APIs from various sources in order to complete the user's task. Specifically, we consider two significant challenges in multiple APIs: \textit{1) graph structures:} some APIs can be executed independently while others need to be executed one by one, resulting in graph-like execution order; and \textit{2) permission constraints:} which source is authorized to execute the API call. We have experimental results on 9 distinct LLMs; e.g., GPT-4o achieves only a 2.0\% success rate at the most complex instruction, revealing that the existing state-of-the-art LLMs still cannot perform well in this situation even with the help of in-context learning and finetuning. Our code and data are publicly available at https://github.com/ruleGreen/AppBench.

==> tables/hir_vs_flat.tex <==
\begin{table}[!t]
%\setlength{\abovecaptionskip}{5pt}   
\setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{adjustbox}{max width=0.48 \textwidth}
    \begin{tabular}{l| ccc|ccc}
    \toprule
    \multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c}{\textbf{
    SS}}  & \multicolumn{3}{|c}{\textbf{SM}} \\    
    % dynamic / multi-turn?
    \cline{2-7} & $F1_{app}$ & $F1_{api}$ & CIFR & $F1_{app}$ & $F1_{api}$ & CIFR \\
    \hline
    GPT-3.5 & 63.60 & 57.95 & 30.81 & 41.49 & 43.65 & 6.50 \\
    \textit{w/ flat }& 50.47 & 44.49 & 16.16 & 12.00 & 31.87 & 1.00 \\
    
    GPT-4o & 88.31 & 86.87 & 70.92 & 50.83 & 50.57 & 20.50 \\
    
    \textit{w/ flat} &89.32 & 93.68 & 77.27 &51.55 &51.29 &18.50 \\
    
    \hdashline
    \multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c}{\textbf{MS}}  & \multicolumn{3}{|c}{\textbf{MM}} \\  
    \cline{2-7} & $F1_{app}$ & $F1_{api}$ & CIFR & $F1_{app}$ & $F1_{api}$ & CIFR \\
    \hline
    GPT-3.5 & 33.17 & 34.53 & 7.00 & 27.79 & 28.09 & 1.00 \\
    \textit{w/ flat} & 7.00 & 22.06 & 2.50 & 6.50 & 22.94 & 0.50 \\
    
    GPT-4o & 39.39 & 39.14 & 11.00 & 32.36 & 32.35 & 2.00 \\
    \textit{w/ flat} & 40.53 & 40.33 & 18.00 & 32.57 & 32.45 & 2.50\\
    
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{The main results of using \textbf{multiple} apps with diversified API usage on \texttt{AppBench}. 
    Bold highlights the best score among all models, and underline underscores the best score under the same model scale}
    \label{tab:hir_vs_flat}
\end{table}

==> tables/multiple_main_exp.tex <==
\begin{table}[!t]
%\setlength{\abovecaptionskip}{5pt}   
\setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{adjustbox}{max width=0.48 \textwidth}
    \begin{tabular}{l| ccc|ccc}
    \toprule
    \multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c}{\textbf{MS}}  & \multicolumn{3}{|c}{\textbf{MM}} \\    
    % dynamic / multi-turn?
    \cline{2-7} & $F1_{app}$ & $F1_{api}$ & CIFR & $F1_{app}$ & $F1_{api}$ & CIFR \\
    \hline
     Mistral-7B & 33.72 & 6.42 & 0.0 & 28.92 & 7.56 & 0.0 \\
     Vicuna-13B & \\
    \hdashline
    
    LLaMA3-8B & 30.65 & 19.52 & 0.10 & 26.39 & 17.80 & 0.05  \\
    LLaMA3-70B & 32.61 & 32.96 & 2.50 & 28.97 & 28.53 & 0.50\\
    
    \hdashline
    QWen1.5-7B & 23.24 & 10.11 & 0.00 & 23.76 & 11.55 & 0.00   \\
    
    QWen1.5-14B & 42.22 & 21.98 & 0.80 &32.62 & 15.07 & 0.00 \\
    QWen1.5-72B & 45.94 & 13.42 & 0.62 & 38.53 & 11.51 & 0.00\\
    
    \hdashline
    
    GPT-3.5 & 33.17 & 34.53 & 7.00 & 27.79 & 28.09 & 1.00 \\
    GPT-4o & 39.39 & 39.14 & 11.00 & 32.36 & 32.35 & 2.00 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{The main results of using \textbf{multiple} apps with diversified API usage on \texttt{AppBench}. 
    Bold highlights the best score among all models, and underline underscores the best score under the same model scale}
    \label{tab:multiple_main_exp}
\end{table}

==> tables/single_main_exp.tex <==
\begin{table}[!t]
%\setlength{\abovecaptionskip}{5pt}   
\setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{adjustbox}{max width=0.48 \textwidth}
    \begin{tabular}{l| ccc|ccc}
    \toprule
    \multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c}{\textbf{SS}}  & \multicolumn{3}{|c}{\textbf{SM}} \\    
    % dynamic / multi-turn?
    \cline{2-7} & $F1_{app}$ & $F1_{api}$ & CIFR & $F1_{app}$ & $F1_{api}$ & CIFR \\
    \hline
    Mistral-7B & 55.97 & 16.31 & 0.51 & 36.59 & 15.09 & 0.50 \\
    Vicuna-13B & 43.20 & 3.70 & 2.00 & \\
    \hdashline
    
    LLaMA3-8B & 63.04 & 42.67 & 23.23 & 37.20 & 25.33 & 0.50 \\
    LLaMA3-70B & 71.20 & 70.00 & 50.00 & 46.48 & 46.96 & 10.50\\
    
    \hdashline
    QWen1.5-7B & 48.14 & 19.54 & 0.00 & 30.13 & 16.71 & 0.00  \\
    
    QWen1.5-14B & 72.89 & 28.41 & 10.10 & 41.89 & 25.51 & 1.50  \\
    QWen1.5-72B & 81.23 & 24.28 & 12.50 & 51.89 & 25.27 & 1.00 \\

    
    \hdashline
    
    GPT-3.5 & 63.60 & 57.95 & 30.81 & 41.49 & 43.65 & 6.50 \\
    GPT-4o & 88.31 & 86.87 & 70.92 & 50.83 & 50.57 & 20.50 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{The main results of \textbf{single} app on \texttt{AppBench}. Bold highlights the best score among all models, and underline underscores the best score under the same model scale}
    \label{tab:single_main_exp}
\end{table}
